Geometric Fabrics: a Safe Guiding Medium for Policy Learning

Robotics policies are always subjected to complex, second order dynamics that entangle their actions with resulting states. In reinforcement learning (RL) contexts, policies have the burden of deciphering these complicated interactions over massive amounts of experience and complex reward functions to learn how to accomplish tasks. Moreover, policies typically issue actions directly to controllers like Operational Space Control (OSC) or joint PD control, which induces straightline motion towards these action targets in task or joint space. However, straightline motion in these spaces for the most part do not capture the rich, nonlinear behavior our robots need to exhibit, shifting the burden of discovering these behaviors more completely to the agent. Unlike these simpler controllers, geometric fabrics capture a much richer and desirable set of behaviors via artificial, second order dynamics grounded in nonlinear geometry. These artificial dynamics shift the uncontrolled dynamics of a robot via an appropriate control law to form behavioral dynamics. Behavioral dynamics unlock a new action space and safe, guiding behavior over which RL policies are trained. Behavioral dynamics enable bang-bang-like RL policy actions that are still safe for real robots, simplify reward engineering, and help sequence real-world, high-performance policies. We describe the framework more generally and create a specific instantiation for the problem of dexterous, in-hand reorientation of a cube by a highly actuated robot hand.

==> sections/02_related_work.tex <==
\section{Related Work}
\label{sec:RelatedWork}
Study of geometry, geometric fabrics.

Notion of forcing the real dynamical system to follow a fictitious one: cover DMPs, RMP does this too

OSC and joint PD control. what the geometry of commands do then. straight lines in end-effector space, straight lines in joint space. 

optimal control, reinforcement learning

talk about problems with existing RL approaches, including complex reward engineering, and robot chatter as a product of policy action noise. Application of ad-hoc low-pass filters (cite dextreme and jason peng's jumping paper), however these introduce phase lag and don't handle joint constraints precisely.

connect with rmp RL policy learning paper by Anqi.

reinforcement learning and issues
1) smoothness
2) complex cost functions
3) better guarantees on stability of behavior

introduce second-order models and geometric fabrics as the most interesting candidate to study
Lots of work on modeling with second order systems. We focus on geometric fabric as it retains the design flexibiltiy of RMPs while remaining stable and emphasizes geometric behavior. Geometric fabrics paper shows improvement over RMPs. We also see that FGPs outperform a variety of baselines as well, including DMP and RMP. Here we use an even broader family of geometric fabrics that makes design easier while retaining stability.


Exploiting the geometry of the fabric via damping levels led to huge boosts in perf.


Need to sequence high performance skills. Existing analytical methods can only go so far due to simplifying assumptions and limimits to our ability to design these. online RL in simulation is promising with strong exhibitions of sim2real on complex manipulation embodiements and tasks. However, complex reward engineering and locality of optimization can impede achieving max perf. Shifting the dynamics of the robot via well understood artificial second order models, in particular, geometric fabric can inject prior knowledge into the behavior in closed form, handle constraints, smoothness, stability, and encourage path consistency. This paradigm has been applied to dexterous in-hand manipulation of a cube, shattering previous levels of performance in real.
